Measurements of the CKM angle beta in charmless loop-dominated B meson decays at BaBar

We report on preliminary measurements of time-dependent CP-violation asymmetries in charmless neutral B meson decays to K+K-K0 (including resonant decays phiK0 and f0K0), eta'K0, pi0K0s, K0sK0sK0s, K0sK0s, rho0K0s, omegaK0s. The results are obtained from a data sample of up to 347 million BBbar pairs produced by e+e- annihilation at the Y(4S) resonance collected with the BaBar detector at the PEP-2 asymmetric-energy B-meson Factory at SLAC.

==> definitions.tex <==

\RequirePackage{xspace}

\usepackage{relsize}
\def\babar{\mbox{\slshape B\kern-0.1em{\smaller A}\kern-0.1em
    B\kern-0.1em{\smaller A\kern-0.2em R}}}

\def\CP                {\ensuremath{C\!P}\xspace}
\def\stwob{\ensuremath{\sin\! 2 \beta   }\xspace}
\def\btos    {\ensuremath{b \to s}\xspace}
\def\btod    {\ensuremath{b \to d}\xspace}
\def\ssbar {\ensuremath{s\overline s}\xspace}
\def\btosss    {\ensuremath{b \to \ssbar s}\xspace}

\def\piz   {\ensuremath{\pi^0}\xspace}
\def\pip   {\ensuremath{\pi^+}\xspace}
\def\pim   {\ensuremath{\pi^-}\xspace}
\def\Kp    {\ensuremath{K^+}\xspace}
\def\Km    {\ensuremath{K^-}\xspace}
\def\KpKm  {\ensuremath{\Kp \kern -0.16em \Km}\xspace}
\def\KS    {\ensuremath{K^0_{\scriptscriptstyle S}}\xspace}
\def\KL    {\ensuremath{K^0_{\scriptscriptstyle L}}\xspace}
\def\Kz    {\ensuremath{K^0}\xspace}
\def\Kzb   {\ensuremath{\Kbar^0}\xspace}
\def\KzKzb {\ensuremath{\Kz \kern -0.16em \Kzb}\xspace}
\def\rhoz   {\ensuremath{\rho^0}\xspace}

\def\Bbar    {\kern 0.18em\overline{\kern -0.18em B}{}\xspace}
\def\Bb      {\ensuremath{\Bbar}\xspace}
\def\BB      {\ensuremath{B\Bbar}\xspace}
\def\Bz      {\ensuremath{B^0}\xspace}
\def\Bzb     {\ensuremath{\Bbar^0}\xspace}
\def\BzBzb   {\ensuremath{\Bz {\kern -0.16em \Bzb}}\xspace}
\def\qqbar {\ensuremath{q\overline q}\xspace}

\def\epem       {\ensuremath{e^+e^-}\xspace}

\mathchardef\Upsilon="7107
\def\Y#1S{\ensuremath{\Upsilon{(#1S)}}\xspace}% no space before {...}!
\def\FourS {\Y4S}

\def\pep2{PEP-II}
\def\deltat{\ensuremath{{\rm \Delta}t}\xspace}
\def\deltamd{\ensuremath{{\rm \Delta}m_d}\xspace}
\providecommand{\dt}{\deltat}

\def\mes        {\mbox{$m_{\rm ES}$}\xspace}
\providecommand{\pvec}{{\bf p}}
\providecommand{\half}{\mbox{${1\over2}$}}

\newcommand{\etal}{{\em et al.}}

\newcommand{\gev}{\ensuremath{\mathrm{\,Ge\kern -0.1em V}}\xspace}
\newcommand{\gevcc}{\ensuremath{{\mathrm{\,Ge\kern -0.1em V\!/}c^2}}\xspace}
\newcommand{\ttag}{\ensuremath{t_{\rm tag}}}
\newcommand{\tcp}{\mbox{$t_{\CP}$}}
\newcommand{\thetaT}{\ensuremath{\theta_{\rm T}}}
\newcommand{\xf}{\mbox{${\cal F}$}}

\newcommand{\etapr}{\ensuremath{\eta^{\prime}}\xspace}

\newcommand{\phikz}{\ensuremath{\phi \kern -0.16em \Kz}\xspace}
\newcommand{\fzkz}{\ensuremath{f_0(980) \kern -0.16em \Kz}\xspace}
\newcommand{\kpkmkz}{\ensuremath{\KpKm \kern -0.16em \Kz}\xspace}
\newcommand{\etaprkz}{\ensuremath{\etapr \kern -0.16em \Kz}\xspace}
\newcommand{\pizkzs}{\ensuremath{\piz \kern -0.16em \KS}\xspace}
\newcommand{\kzskzskzs}{\ensuremath{\KS\KS\KS}\xspace}
\newcommand{\kzskzs}{\ensuremath{\KS\KS}\xspace}
\newcommand{\rhozkzs}{\ensuremath{\rhoz \kern -0.16em \KS}\xspace}
\newcommand{\omegakzs}{\ensuremath{\omega \kern -0.16em \KS}\xspace}

\newcommand{\btokzskzs}{\ensuremath{\Bz \to \KS\KS}\xspace}

\newcommand{\msp}{\ensuremath{\phantom{-}}}
\newcommand{\PM}{\ensuremath{\kern -0.21em\pm\kern -0.21em}\xspace}

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: t
%%% End: 

